Online Feature Updates Improve Online (Generalized) Label Shift Adaptation

This paper addresses the prevalent issue of label shift in an online setting with missing labels, where data distributions change over time and obtaining timely labels is challenging. While existing methods primarily focus on adjusting or updating the final layer of a pre-trained classifier, we explore the untapped potential of enhancing feature representations using unlabeled data at test-time. Our novel method, Online Label Shift adaptation with Online Feature Updates (OLS-OFU), leverages self-supervised learning to refine the feature extraction process, thereby improving the prediction model. By carefully designing the algorithm, theoretically OLS-OFU maintains the similar online regret convergence to the results in the literature while taking the improved features into account. Empirically, it achieves substantial improvements over existing methods, which is as significant as the gains existing methods have over the baseline (i.e., without distribution shift adaptations).

==> sections/algorithms.tex <==
% ORIGINAL ALGORITHM
\begin{comment}
\begin{algorithm}[!t]
\caption{Revised ROGD for online feature updates ROGD-R. See the original version in Equation 7 and Equation 8 in \cite{wu2021online}.}
\begin{algorithmic}
	\STATE \textbf{Require:} Learning rate $\eta$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$, the training label marginal $q_0:=\calP^{\rm train}(y)$.
%		\STATE 1. Grab the neural network $f_t''$ that $f_t$ is reweighting of.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: $s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{red}f_{t}''}, D_0'}{\color{red}f_{t}''}(x_t)$. \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original ROGD, it is $f_0$ rather than $f_t$.}
		\STATE 2. Grab the weight $p_t$ from $f_t$.
		\STATE 3. Update $p_{t+1}:= {\rm Proj}_{\Delta^{K-1}}\left[p_t - \eta\cdot J_{p}(p_t)^{\top}s_t\right]$, where $J_{p, {\color{red}f_{t}''}}(p_t) = \frac{\partial}{\partial p}(1 - {\rm diag}(C_{{\color{red}f_{t}''}, D_0, p}))|_{p = p_{t}}$, and let $f_{t+1}$ be a reweighting version of {\color{red}$f_{t}''$} by the weight $\left(\frac{p_{t+1}[k]}{q_0[k]}: k=1, \cdots K\right)$
		 \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original ROGD, it is $f_0$ rather than $f_{t}''$.}
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_rogd}
\end{algorithm}
\end{comment}
\begin{algorithm}[!t]
\caption{Revised ROGD for online feature updates ROGD-R. See the original version in Equation 7 and Equation 8 in \cite{wu2021online}.}
\begin{algorithmic}
	\STATE \textbf{Require:} Learning rate $\eta$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$, the training label marginal $q_0:=\calP^{\rm train}(y)$.
%		\STATE 1. Grab the neural network $f_t''$ that $f_t$ is reweighting of.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: \\ \phantom{1. C}$s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{anncolor}f_{t}''}, D_0'}{\color{anncolor}f_{t}''}(x_t)$. \phantom{========..} {\color{anncolor} \small $\rhd$ In the original ROGD, it is $f_0$ rather than $f_t$.}
		\STATE 2. Grab the weight $p_t$ from $f_t$.
		\STATE 3. Update $p_{t+1}:= {\rm Proj}_{\Delta^{K-1}}\left[p_t - \eta\cdot J_{p}(p_t)^{\top}s_t\right]$, \\ \phantom{3. }where $J_{p, {\color{anncolor}f_{t}''}}(p_t) = \frac{\partial}{\partial p}(1 - {\rm diag}(C_{{\color{anncolor}f_{t}''}, D_0, p}))|_{p = p_{t}}$, and let $f_{t+1}$ be a reweighting version of \phantom{3. .}{\color{anncolor}$f_{t}''$} by the weight $\left(\frac{p_{t+1}[k]}{q_0[k]}: k=1, \cdots K\right)$
		 \ \ \ \ \ \ \ \ \ {\color{anncolor} \small $\rhd$ In the original ROGD, it is $f_0$ rather than $f_{t}''$.}
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_rogd}
\end{algorithm}

% ORIGINAL ALGORITHM
\begin{comment}
\begin{algorithm}[!t]
\caption{Revised FTH for online feature updates (FTH-R). See the original version in Equation 9 in \cite{wu2021online}.}
\begin{algorithmic}
%	\STATE \textbf{Require:}
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$; the training label marginal $q_0:=\calP^{\rm train}(y)$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: $s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{red}f_{t}}, D_0'}{\color{red}f_{t}''}(x_t)$. \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original FTL, it is $f_0$ rather than $f_t''$.}
		\STATE 2. Compute $p_{t+1}=\frac{1}{t}\sum_{\tau=1}^ts_{\tau}$
		\STATE 3. Let $f_{t+1}$ be a reweighting version of {\color{red}$f_{t}''$} by the weight $\left(\frac{p_{t+1}[k]}{q_0[k]}: k=1, \cdots K\right)$
		 \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original FTL, it is $f_0$ rather than $f_{t}''$.}
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_fth}
\end{algorithm}
\end{comment}
\begin{algorithm}[!t]
\caption{Revised FTH for online feature updates (FTH-R). See the original version in Equation 9 in \cite{wu2021online}.}
\begin{algorithmic}
%	\STATE \textbf{Require:}
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$; the training label marginal $q_0:=\calP^{\rm train}(y)$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: \\ \phantom{1. }$s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{anncolor}f_{t}}, D_0'}{\color{anncolor}f_{t}''}(x_t)$. \phantom{===========.} {\color{anncolor} \small $\rhd$ In the original FTL, it is $f_0$ rather than $f_t''$.}
		\STATE 2. Compute $p_{t+1}=\frac{1}{t}\sum_{\tau=1}^ts_{\tau}$
		\STATE 3. Let $f_{t+1}$ be a reweighting version of {\color{anncolor}$f_{t}''$} by \\ \phantom{3. }the weight $\left(\frac{p_{t+1}[k]}{q_0[k]}: k=1, \cdots K\right)$ \phantom{==========}{\color{anncolor} \small $\rhd$ In the original FTL, it is $f_0$ rather than $f_{t}''$.}
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_fth}
\end{algorithm}

% ORIGINAL ALGORITHM
\begin{comment}
\begin{algorithm}[!t]
\caption{Revised UOGD for online feature updates (UOGD-R). See the original version in Equation 9 in \cite{bai2022adapting}.}
\begin{algorithmic}
	\STATE \textbf{Require:} The learning rate $\eta$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, initial classifier $f_0$, the validation set $D_0'$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: $s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{red}f_{t}''}, D_0'}{\color{red}f_{t}''}(x_t)$. \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original UOGD, it is $f_0$ rather than $f_t$.}
		\STATE 2. Grab the weight $w_t$ from the last linear layer of $f_t$.
		\STATE 3. Update $w_{t+1}:= w_t - \eta\cdot \frac{\partial}{\partial w} J_{w}(w_t)^{\top}s_t$, where $J_{w}(w_t) = \frac{\partial}{\partial w}(\hat{R}_t^1(w), \cdots, \hat{R}_t^K(w))|_{w = w_{t}}$, 
		$\hat{R}_t^k(w)=\frac{1}{|D_0^k|}\sum_{(x, y)\in D_0^k}\ell_{\rm ce}(f(x|{\color{red}\theta^{\rm feat}_{t}}, \theta^{\rm linear}=w), y)$, $D_0^k$ denotes the set of data with label $k$ in $D_0$. 		 \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original UOGD, it is $\theta^{\rm feat}_{0}$ rather than ${\color{red}\theta^{\rm feat}_{t}}$.}
		
		\STATE 4. Let $f_{t+1}$ be $f(\cdot|\theta^{\rm feat}_{t}, w_{t+1})$.
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_uogd}
\end{algorithm}
\end{comment}
\begin{algorithm}[!t]
\caption{Revised UOGD for online feature updates (UOGD-R). See the original version in Equation 9 in \cite{bai2022adapting}.}
\begin{algorithmic}
	\STATE \textbf{Require:} The learning rate $\eta$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, initial classifier $f_0$, the validation set $D_0'$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: \\ \phantom{1.} $s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{anncolor}f_{t}''}, D_0'}{\color{anncolor}f_{t}''}(x_t)$. \phantom{==========.}{\color{anncolor} \small $\rhd$ In the original UOGD, it is $f_0$ rather than $f_t$.}
		\STATE 2. Grab the weight $w_t$ from the last linear layer of $f_t$.
		\STATE 3. Update $w_{t+1}:= w_t - \eta\cdot \frac{\partial}{\partial w} J_{w}(w_t)^{\top}s_t$, where $J_{w}(w_t) = \frac{\partial}{\partial w}(\hat{R}_t^1(w), \cdots, \hat{R}_t^K(w))|_{w = w_{t}}$, 
		\\ \phantom{3.} $\hat{R}_t^k(w)=\frac{1}{|D_0^k|}\sum_{(x, y)\in D_0^k}\ell_{\rm ce}(f(x|{\color{anncolor}\theta^{\rm feat}_{t}}, \theta^{\rm linear}=w), y)$, $D_0^k$ denotes the set of data with \\ \phantom{3. }label $k$ in $D_0$. \phantom{=====================} {\color{anncolor} \small $\rhd$ In the original UOGD, it is $\theta^{\rm feat}_{0}$ rather than ${\color{anncolor}\theta^{\rm feat}_{t}}$.}
		
		\STATE 4. Let $f_{t+1}$ be $f(\cdot|\theta^{\rm feat}_{t}, w_{t+1})$.
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_uogd}
\end{algorithm}

% ORIGINAL ALGORITHM
\begin{comment}
\begin{algorithm}[!t]
\caption{Revised ATLAS for online feature updates (ATLAS-R). See the original version in Equation 9 in \cite{bai2022adapting}.}
\begin{algorithmic}
	\STATE \textbf{Require:} The learning rate pool $\calH$ with size N; Meta learning rate $\varepsilon$; $\forall i\in[N]$, $p_{1, i}=1/N$ and $w_{1, i}=\theta^{\rm linear}_{f_0}$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: $s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{red}f_{t}}, D_0'}{\color{red}f_{t}''}(x_t)$. \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original ATLAS, it is $f_0$ rather than $f_t''$.}
		\FOR{$i\in [N]$}
		\STATE 2. Update $w_{t+1, i}:= w_{t, i} - \eta_i\cdot \frac{\partial}{\partial w} J_{w}(w_{t, i})^{\top}s_t$, where $J_{w}(w_{t, i}) = \frac{\partial}{\partial w}(\hat{R}_t^1(w), \cdots, \hat{R}_t^K(w))|_{w = w_{t, i}}$, 
		$\hat{R}_t^k(w)=\frac{1}{|D_0^k|}\sum_{(x, y)\in D_0^k}\ell_{\rm ce}(f(x|{\color{red}\theta^{\rm feat}_{t}}, w), y)$, $D_0^k$ denotes the set of data with label $k$ in $D_0$. 		 \ \ \ \ \ \ \ \ \ {\color{red} $\backslash\backslash$ In the original ATLAS, it is $\theta^{\rm feat}_{0}$ rather than $\theta^{\rm feat}_{t}$.}
		\ENDFOR
		\STATE 3. Update weight $p_{t+1}$ according to $p_{p_{t, i}}\propto \exp(-\varepsilon\sum_{\tau=1}^{t-1}\hat{R}_{\tau}(\bw_{\tau, i}))$
		\STATE 3. Compute $w_{t+1}=\sum_{i=1}^Np_{t+1, i}w_{t+1, i}$. Let $f_{t+1}$ be $f(\cdot|\theta^{\rm feat}_{t}, w_{t+1})$.
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_atlas}
\end{algorithm}
\end{comment}
\begin{algorithm}[!t]
\caption{Revised ATLAS for online feature updates (ATLAS-R). See the original version in Equation 9 in \cite{bai2022adapting}.}
\begin{algorithmic}
	\STATE \textbf{Require:} The learning rate pool $\calH$ with size N; Meta learning rate $\varepsilon$; $\forall i\in[N]$, $p_{1, i}=1/N$ and $w_{1, i}=\theta^{\rm linear}_{f_0}$.
	\FOR{$t=1, \cdots, T$}
		\STATE \textbf{Input at time $t$:} Samples $S_t$ and model $f_{t}$ at time $t$, previous samples $S_1\cup\cdots\cup S_{t-1}$, previous models $\{f_1, \cdots, f_{t-1}\}$ and $\{f_1'', \cdots, f_{t}''\}$ from step 3 in Algorithm~\ref{alg:ols_feu}, the validation set $D_0'$.
		\STATE 1. Compute the unbiased estimator for label marginal distribution: \\ \phantom{1. }$s_t=\frac{1}{|S_t|}\sum_{x_t\in S_t} C^{-1}_{{\color{anncolor}f_{t}}, D_0'}{\color{anncolor}f_{t}''}(x_t)$. \phantom{=========.} {\color{anncolor} \small $\rhd$ In the original ATLAS, it is $f_0$ rather than $f_t''$.}
		\FOR{$i\in [N]$}
		\STATE 2. Update $w_{t+1, i}:= w_{t, i} - \eta_i\cdot \frac{\partial}{\partial w} J_{w}(w_{t, i})^{\top}s_t$, where \\ 
          \phantom{1. }$J_{w}(w_{t, i}) = \frac{\partial}{\partial w}(\hat{R}_t^1(w), \cdots, \hat{R}_t^K(w))|_{w = w_{t, i}}$, \\
		\phantom{1. }$\hat{R}_t^k(w)=\frac{1}{|D_0^k|}\sum_{(x, y)\in D_0^k}\ell_{\rm ce}(f(x|{\color{anncolor}\theta^{\rm feat}_{t}}, w), y)$, $D_0^k$ denotes the set of data \\ \phantom{1. }with label $k$ in $D_0$.  \phantom{================}{\color{anncolor} \small $\rhd$ In the original ATLAS, it is $\theta^{\rm feat}_{0}$ rather than $\theta^{\rm feat}_{t}$.}
		\ENDFOR
		\STATE 3. Update weight $p_{t+1}$ according to $p_{p_{t, i}}\propto \exp(-\varepsilon\sum_{\tau=1}^{t-1}\hat{R}_{\tau}(\bw_{\tau, i}))$
		\STATE 3. Compute $w_{t+1}=\sum_{i=1}^Np_{t+1, i}w_{t+1, i}$. Let $f_{t+1}$ be $f(\cdot|\theta^{\rm feat}_{t}, w_{t+1})$.
		 \STATE \textbf{Output at time $t$:} $f_{t+1}$.
	\ENDFOR	
\end{algorithmic}
\label{alg:rv_atlas}
\end{algorithm}


==> sections/exp_setup.tex <==
\section{Further experiment details}

The configurations used for experiments are listed below.

(Train) CIFAR-10, CINIC, STL10
\begin{itemize}
    \item dataset: CIFAR-10, CINIC, STL10
    \item model: ResNet18 (groupnorm)
    \item method: Test-Time Training (TTT), TENT \rw{Can you rename it as Rotation Degree Prediction and Entropy Minimization? Keep the consistency as the main text!}
    \item epochs: 70
    \item batch size: 200
    \item learning rate: 0.1
    \item momentum: 0.9
    \item weight decay: 0.0001
    \item seed: 4242
    \item loss: cross entropy
    \item scheduler: gamma=0.1, milestones at 25th and 40th epoch
    \item optimizer: SGD
\end{itemize}

(Train) EUROSAT
\begin{itemize}
    \item dataset: EUROSAT
    \item model: ResNet18 (groupnorm)
    \item method: Test-Time Training (TTT), TENT
    \item epochs: 50
    \item batch size: 200
    \item learning rate: 0.1
    \item momentum: 0.9
    \item weight decay: 0.0001
    \item seed: 4242
    \item loss: cross entropy
    \item scheduler: gamma=0.1, milestones at 25th and 40th epoch
    \item optimizer: SGD
\end{itemize}

(Eval) CIFAR-10, CINIC, STL10, EUROSAT
\begin{itemize}
    \item total time: 1000
    \item shift type: monotone, sinusoidal, bernouli
    \item up-to-date BBSE: true
    \item number of online samples: 10
    \item seed: 8610
    \item using current marginal estimate: false
    \item use default ROGD lipschitz: true
    \item learning rate: 0.1
    \item momentum: 0.9
    \item weight decay: 0.0001
    \item optimizer: SGD
\end{itemize}

(Eval) CIFAR-10C
\begin{itemize}
    \item corruption types (severity): gaussian noise (), brightness (), fog (), pixelate ()
    \item total time: 1000
    \item shift type: monotone, sinusoidal, bernouli
    \item up-to-date BBSE: true
    \item number of online samples: 10
    \item seed: 8610
    \item using current marginal estimate: false
    \item use default ROGD lipschitz: true
    \item learning rate: 0.1
    \item momentum: 0.9
    \item weight decay: 0.0001
    \item optimizer: SGD
\end{itemize}


\begin{comment}
Changing order of prediction/update
\begin{itemize}
    \item 
\end{itemize}

Consistency between online/offline method used
\begin{itemize}
    \item 
\end{itemize}

Ablation - domain shift
\begin{itemize}
    \item 
\end{itemize}

Ablation - batch accumulation / other SSL methods (simclr, MoCo)
\begin{itemize}
    \item 
\end{itemize}

Ablation - pseudo-labelling / self-training 
\begin{itemize}
    \item 
\end{itemize}

\end{comment}



==> sections/experiment.tex <==
\section{Experiment}
\label{sec:exp}
\begin{figure*}[!t]
\centering
\includegraphics[width=0.85\linewidth]{figs/main_results.pdf}
%\vspace{-3ex}
\caption{Evaluation of OLS and OLS-OFU.} 
% bring the text back if more text is needed (a). OLS-OFU when paired with three different SSL methods consistently performs better than OLS on CIFAR-10 for online label shift; (b). The improvement becomes more significant on generalized online label shift, under three types of domain shift.
\label{fig:main_results}
%\vspace{-3ex}
\end{figure*}

In this section, we empirically evaluate how OLS-OFU improves the original OLS methods on both online label shift and online generalized label shift\footnote{Code released at {\tiny \url{https://anonymous.4open.science/r/online_label_shift_with_online_feature_updates-3A1F/}}.}.
The experiment is performed on CIFAR-10~\citep{krizhevsky2009learning}, STL10 \citep{coates2011stl10}, CINIC \citep{darlow2018cinic10}, and EuroSAT \citep{8736785} for testing online label shift, and CIFAR-10C~\citep{hendrycks2019benchmarking} for testing online generalized label shift. We systematically vary the distribution shift processes and 
% semi-supervised learning (SSL) 
self-supervised learning (SSL) 
techniques to assess the effectiveness of the proposed method.

\subsection{Experiment Set-up}
\textbf{Dataset and Label Shift Settings.}
For online label shift, we evaluate the efficacy of our algorithm on CIFAR-10 \citep{krizhevsky2009learning}, STL10 \citep{coates2011stl10}, CINIC \citep{darlow2018cinic10}, and EuroSAT \citep{8736785}, which have 10 categories of images.
For each dataset, we split the original train set into the offline train (i.e., $D_0$) and validation sets (i.e., $D'_0$) following a ratio of $4:1$.
%, which have 40,000 and 10,000 images respectively.
At the online test unlabeled batches are sampled from the test set.
% of CIFAR-10.
For online generalized label shift, the offline train and validation sets are the same CIFAR-10 images.  The test unlabeled batches are drawn from CIFAR-10C, a benchmark with the same objects as CIFAR-10 but with various types of corruption.
We experiment with three types of corruptions with CIFAR-10C: Gaussian noise, Fog and Pixelate.
%Besides CIFAR-10 and CIFAR-10C, we also experiment with three additional datasets for the setting of online label shift and present the results in Appendix~\ref{sec:app_moredata} due to the space limits.
%See more details of dataset set-up in Appendix~\ref{sec:app_details_data}.
% due to space limit.

We follow \citet{bai2022adapting} and \citet{baby2023online} to simulate the online label distribution shift with two shift patterns: Sinusoidal shift and Bernoulli shift.
Specifically, given two label distribution vectors $q$ and $q'$,
we simulate the label marginal distributions at time $t$ as a weighted combination of them: $q_t:=\alpha_t q + (1-\alpha_t)q'$.
In Sinusoidal shift, $\alpha_t=\sin \frac{i\pi}{L}$ (periodic length $L=\sqrt{T}$, $i=t \textnormal{ mod } L$) while in Bernoulli shift, $\alpha_t$ is a random bit (either 0 or 1), 
where the bit switches $\alpha_t=1-\alpha_{t-1}$ with probability $p=1-\frac{1}{\sqrt{T}}$.
In our experiments, we set the initial distribution vector $q$ and $q'$ with $\frac{1}{K}(1, \cdots, 1)$ and $(1, 0, \cdots, 0)$.
To sample the batch test data at time $t$, we first sample a batch of labels (not revealed to the learner) according to $q_t$. Then given each label we can sample an image from the test set, and collect this batch of images without labels as $S_t$.
We experiment with $T=1000$ and batch size $B=10$ at each time step, following \citet{baby2023online}.

\textbf{Evaluation Metric.}
We report the average error during test, i.e., $\frac{1}{TB}\sum_{t=1}^T\sum_{x_t\in S_t}\mathbbm{1}\left( f_t(x_t) \neq y_t \right)$, where $(x_t, y_t)\sim \calP_t^{\rm test}$, to approximate $\frac{1}{T}\sum_{t=1}^T \ell(f_t; \calP^{\rm test}_t)$ for the evaluation efficiency. 
This is valid for large $T$ due to its exponential concentration rate by the Azuma–Hoeffding inequality.

\textbf{Self-supervised learning. }
In the experiment, we narrow our focus on three particular SSL techniques in the evaluation for classification tasks: rotation degree prediction~\citep{gidaris2018unsupervised, sun2020test}, entropy minimization~\citep{grandvalet2004semi, wang2020tent} and MoCo~\citep{he2020momentum, chen2020mocov2, 9711302}. 
It is important to note that this concept extends beyond these three SSL techniques, and the incorporation of more advanced SSL techniques has the potential to further elevate the performance.
Specifically, rotation degree prediction 
involves initially rotating a given image by a specific degree from the set $\{0, 90, 180, 270\}$ and the classifier is required to determine the degree by which the image has been rotated. 
Entropy minimization utilizes a minimum entropy regularizer, with the motivation that unlabeled examples are mostly beneficial when classes have a small overlap.
MoCo is a more advanced representation learning technique, 
using a query and momentum encoder to learn representations from unlabeled data by maximizing the similarity of positive pairs and minimizing the similarity of negative pairs.
More details of these SSL techniques are given in Appendix~\ref{sec:app_ssl_details}.

\textbf{Baselines and OLS Methods.}
We perform an extensive evaluation of 6 OLS methods in the literature: FTFWH, FTH, ROGD, UOGD, ATLAS, and FLHFTL.
% FTFWH is an empirical OLS proposed in \citet{wu2021online}. \yi{why we only mention FTFWH here? either we delete this sentence or introduce others as well?}
We further report the performance of our method OLS-OFU (Algorithm~\ref{alg:ols_feu}) applied on top of each OLS. OLS-OFU is instantiated with 3 common SSL methods introduced in Section~\ref{sec: ps}: rotation degree prediction, entropy minimization, and MoCo.
We run the batch accumulation variant of Algorithm~\ref{alg:ols_feu} for MoCo and set BA=$50$; please see the ablation for the selection of BA in Appendix~\ref{app:batch_acc}.
Additionally, we report two baseline scores, Base and OFU. 
The Base uses the fixed pre-trained model $f_0$ to predict the labels at all time steps.
The second is online feature updates (OFU) only, where at time step $t$ we only update the features (Step 2 in Algorithm~\ref{alg:ols_feu}) without utilizing OLS algorithms.

\subsection{Results }
% \textbf{Main results on CIFAR-10 and CIFAR-10C.}
\textbf{Main Results: comparison between OLS-OFU and baselines under online (generalized) label shift.} 
Figure~\ref{fig:main_results}(a) shows the performance comparison between OLS-OFU, implemented with \textit{three SSL methods}, and their corresponding OLS counterparts on CIFAR-10 under the scenario of \emph{classical online label shift}.
Figure~\ref{fig:main_results}(b) shows the results on \textit{three more datasets} with SSL technique in OLS-OFU being rotation degree prediction.
The online shift pattern in the setting of Figure~\ref{fig:main_results}(a-b) is sinusoidal shift.
% Figure~\ref{fig:main_results}(a) presents the results of Sinusoidal shift on CIFAR-10, which evaluates the algorithms for online label shift. The results include 3 SSL methods in OLS-OFU.
From Figure~\ref{fig:main_results}(a-b), we can observe that OLS-OFU outperforms all other baselines.
Notably, OLS-OFU, when integrated with three SSL methods, consistently outperforms their counterpart OLS method across all of the OLS methods.
This emphasizes the importance of improving representation learning within label shift adaptation and underscores the robustness of our framework OLS-OFU.
Results for Bernoulli shift in Appendix~\ref{sec:app_cifar10} show similar conclusion.

%, both OLS and OLS-OFU show significantly better performance than Base and OFU. 
%This demonstrates the inherent advantages of OLS methods in effectively addressing the online label shift problem.
% This implies that in the online label shift problem OLS methods have certain advantages to tackle this specific problem.
%Additionally, it's worth noting that OLS-OFU, when integrated with three distinct SSL methods, consistently outperforms OLS across all six OLS methods.
% Moreover, OLS-OFU within 3 SSL methods are consistently better than OLS for all 6 OLS methods.
%This underscores the importance of improving feature representation learning within label shift adaptation in OLS-OFU.
%We have the similar conclusion to the CIFAR-10 results.
%Results for Bernoulli shift in Appendix~\ref{sec:app_cifar10} show similar conclusion.

% , while also highlighting the effectiveness of the OLS-OFU framework.
% This validates the improvements when we carefully adapt online feature updates into OLS. 
% Appendix~\ref{sec:app_cifar10} shows similar conclusions for other types of distribution shift as well, such as the Bernoulli shift.
 

Furthermore, we report the performance of OLS-OFU in the context of \textit{online generalized label shift}. In this scenario, the test images exhibit three types of domain shifts in CIFAR-10C --- Gaussian noise, Fog, and Pixelation—with mild severity. 
We present the result under Sinusoidal shift with the SSL method used in OLS-OFU as rotation degree prediction.
Similar to the scenario of online label shift, the superior performance of OLS-OFU compared with Base, OFU, and OLS demonstrates its superiority (Figure~\ref{fig:main_results}(c)).
Particularly, OLS-OFU consistently outperforms the original OLS methods by an even larger gap than the one occurring at the classic label shift setting.
We hypothesize that the inclusion of SSL methods within OLS-OFU aids the learning of the unknown mapping $h$ inherent in the generalized label shift assumption. 
As evaluated in~\citet{sun2020test}, the label shift assumption in the feature space of $\theta^{\rm feat}_t$ is violated milder than the one of $\theta^{\rm feat}_0$ --- the more severe violation of $\theta^{\rm feat}_0$ explains why some OLS methods perform even worse than OFU.
Results for other SSL methods and online shift patterns show a similar pattern in Appendix~\ref{sec:app_cifar10c}.

% Overall, OLS-OFU through various SSL methods achieves the SOTA performance across multiple datasets and online shift patterns. 
% To see the significance, the improvement from the previous state-of-the-art (SOTA) method FLHFTL to FLHFTL-OFU is comparable with and more consistent to the improvements along the previous OLS methods across different data and online shift patterns.
Moreover, as an \textit{ablation study} of OLS-OFU, the comparison between OLS-OFU and either OLS or OFU individually underscores the specific benefits of both the OFU and OLS modules in addressing the challenges posed by the online (generalized) label shift problem.

%As shown in Figure~\ref{fig:main_results}(c), OFU has huge improvements from Base, showing the necessity of updating feature extractors to facilitate the learning of $h$.
%Moreover, some OLS methods perform worse than OFU. This is expected as the underlying assumption of label shift no longer holds in this generalized label shift setting.
%Lastly, it is worth highlighting that OLS-OFU consistently outperforms the original OLS methods by a larger gap than the one occurring at the classic label shift setting. We hypothesize that the SSL methods within OLS-OFU aid the feature extractor in learning the unknown mapping $h$ within the generalized label shift assumption. Intuitively, the label shift assumption in the feature space of $\theta^{\rm feat}_t$ is violated lighter than the one in the feature space of $\theta^{\rm feat}_0$. Given the relatively mild violation, the OLS module within OLS-OFU continues to help adapt the online label shift, explaining OLS-OFU's advantage over OFU.

% Lastly, OLS-OFU outperforms all other methods.
% We hypothesize that the SSL method helps the feature extractor approach the unknown $h$ in the assumption of generalized label shift.
% Then the label shift assumption in the feature space of $\theta^{\rm feat}_t$ is violated much lighter than the one in the feature space of $\theta^{\rm feat}_0$ in OLS. This explains why OLS-OFU is significantly and consistently better than OLS.
% With such a light violation, the OLS module in OLS-OFU still has a positive influence on the results, thus explaining why OLS-OFU outperforms OFU.
% \begin{wrapfigure}{r}{0.55\textwidth}
%     \vspace{-3ex}
%     \begin{minipage}{0.55\textwidth}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\linewidth]{figs/main_regret_sc.pdf}
\caption{Empirical examination for the holdness of Equation~\ref{eq:second_regret}. Clean denotes the experiment on CIFAR-10 and others denotes the corruption type. They are paired with two online shift patterns: Sinusoidal and Bernoulli.}% Gaussion, Fog and Pixelate denote various domain shifts in CIFAR-10C.
\vspace{-3ex}
\label{fig:main_oracle}
\end{figure}
% %\end{figure*}
% \end{minipage}
% \end{wrapfigure}

\textbf{Empirical validation of Equation~\ref{eq:second_regret}.}
In Section~\ref{sec:old-ofu_thm}, we argued that when the inequality in Equation~\ref{eq:second_regret} holds, the loss of FLHFTL-OFU exhibits a tighter upper bound compared to FLHFTL.
Figure~\ref{fig:main_oracle} presents the RHS (corresponds to OLS) and LHS (corresponds to OLS-OFU with SSL loss as rotation degree prediction) of Equation~\ref{eq:second_regret}. We perform the study over eight different settings and varies the domain shift and online shift patterns. It is evident that OLS-OFU yields improvements on the \emph{baseline} of the regret as shown in Equation~\ref{eq:second_regret}.
Appendix~\ref{sec:app_ab3} validates this inequality for other SSL techniques.
We further examine how the improvement from Equation~\ref{eq:second_regret} (RHS - LHS) is correlated the improvement from OLS to OLS-OFU.
For each OLS method, we compute the Pearson coefficient (within the range of [-1, 1]) between these two terms across all experimental setups (varying dataset, online shift pattern, and SSL methods). The calculated coefficients are 0.70, 0.76, 0.54, 0.63, 0.58, and 0.75 when OLS is FTFWH, FTH, ROGD, ATLAS, UOGD, or FLHFTL, respectively. These values indicate strong positive correlations, underscoring how improvements in regret align with empirical performance improvements.

 \textbf{Results on CIFAR-10C with higher severity.}
%\textbf{How does OLS-OFU perform under high severity of domain shift in the setting of generalized online label shift?}
% We also test all methods for the 3 domain shifts but increase their severities.
We evaluate all methods on CIFAR-10C with higher severity of domain shifts. Figure~\ref{fig:main_cifar10c_severe} shows the results when the test images are corrupted by Gaussian noise\footnote{Please refer to Appendix~\ref{sec:app_cifar10c_high} for results involving higher levels of severity, other corruption types, and SSL techniques.}.
Comparing with Figure~\ref{fig:main_results}(c), it is clear that as the severity increases, OLS-OFU enlarges the performance gap compared to OLS.
However, it might be worth pointing out that neither OLS nor OLS-OFU are better than OFU. 
%\begin{wrapfigure}{r}{0.3\textwidth}
%    \begin{minipage}{0.3\textwidth}
\begin{figure}[!t]
\centering
%\vspace{-3ex}
\includegraphics[width=0.5\linewidth]{figs/main_cifar10c_severe.pdf}
\caption{Results on CIFAR-10C for a high level of severity.}
\label{fig:main_cifar10c_severe}
\vspace{-3ex}
 \end{figure}
%\end{minipage}
%\end{wrapfigure}
This is because the severe violation of the label shift assumption --- noted that even OFU cannot reduce the violation under an acceptable level (still get 20$\%$ error rate), which gives inferior performance of OLS-OFU compared to OFU, as the adaptation to distribution shift deviates significantly. %\yi{please check}.

%\textbf{The ablation study of the order of prediction and update.} 
%In the default online distribution shift framework  (Figure~\ref{fig:overview_odsa}), model updates occur after making predictions for samples at timestep $t$. This raises the question of whether the model should be updated before making predictions. We conducted empirical evaluations for both the ``predict first'' and ``update first''  approaches and found no compelling evidence to favor one over the other (additional results in Appendix~\ref{sec:app_ab1}).
%However, it's noteworthy that within the ``predict first'' framework, OLS and OLS-OFU benefit from robust theoretical guarantees, hence we recommend the ``predict first'' approach in practical applications.

==> sections/introduction.tex <==
\section{Introduction}
In the real-world, train data and test data may not share the same distribution \emph{(distribution shift)}.
% 
Prior work focus on distribution shifts in offline or batch settings, where a single shift occurs between the train and test distributions.
In the real-world, test data may arrive in an \emph{online} fashion, the distribution shift may continuously evolve over time, and may suffer from \emph{missing or delayed} labels.
% stemming from the online setup, 
% where gathering labels for the streaming data in a timely manner becomes a challenging task.

%% formulate, and prior work on online label shift
% To tackle the distribution shift problem, prior work makes further assumptions on the nature of the shift, such as label shift or covariate shift. %, or missingness shift~\cite{}. 
We focus on the common \emph{(generalized) label shift} problem in an online fashion with missing labels. Specifically, the learner is given a fixed set of labeled training data $D_0\sim \mathcal{P}^{\rm train}$  and trains a model $f_0$. At test-time, a small batch of unlabelled test data $S_t\sim \mathcal{P}^{\rm test}_{t}$ arrives in an online fashion ($t=1, 2, \cdots$). For online label shift, we assume the label distribution $\mathcal{P}^{\rm test}_{t}(y)$ may change over time $t$ while the conditional distribution  stays the same, i.e. $\mathcal{P}^{\rm test}_{t}(x|y) = \mathcal{P}^{\rm train}(x|y)$. 
% 
MRI image classifiers for concussion detection can be challenging due to label shift caused by seasonal changes in the image distribution. A classifier trained during skiing season may perform poorly when tested afterward, as the image distribution changes continuously between skiing and non-skiing seasons.
% 
The \emph{generalized} label shift relaxes this assumption by assuming there exists a transformation $h$ of the covariate, such that the conditional distribution $\mathcal{P}^{\rm test}_{t}(h(x)|y) = \mathcal{P}^{\rm train}(h(x)|y)$ stays the same.
% , for instance
% Reiterating our example, cameras or 3D laser scanning machines employed in various regions may exhibit disparities in attributes like resolution and contrast, leading to distinct distributions of the same Cacao images. 
% 
The classifier on MRI images can also be used in different clinics during training and testing.
MRI machines differing in hardware and software versions may result in image variations (e.g. brightness, resolution).
% The classifier on MRI images can also be used in different clinics during training and testing, where the MRI machines might have different versions at both hardware and software levels.
% Then, the images may have some variations such as brightness, resolution, etc.
However, a feature extractor $h$ exists, capable of mapping these variations to the same point in the latent space. 
The goal of the learner is to adapt to the (generalized) label shift within the non-stationary environment, continually adjusting the model's predictions in real-time. 

\begin{figure*}[ht]
\includegraphics[width=\linewidth]{figs/problem_setting}
\caption{Overview of online distribution shift adaptation. We further assume $\calP^{\rm test}_t(x|y) = \calP^{\rm train}(x|y)$ for online label shift adaptation and assume the existence of unknown feature transformation $h$ such that  $\calP^{\rm test}_t(h(x)|y) = \calP^{\rm train}(h(x)|y)$ for online generalized label shift adaptation.}
\label{fig:overview_odsa}
\end{figure*}

%% drawbacks of previous approaches, using various examples
Online label shift adaptation (OLS) algorithms primarily adopt one of two strategies: directly reweighting of the pretrained classifier $f_0$, or re-training only the final linear layer of $f_0$.
% --- typically keeping the feature extractor frozen. 
Recent work demonstrates that feature extractors could be improved, even during test-time and in the absence of labels.
We hypothesize that a similar effect can be leveraged in the (generalized) label shift setting and propose to improve the feature representation during testing. 
% In online label shift, 
Updating the feature extractor offers two advantages. 
First, it enables the utilization of additional unlabeled samples to enhance the sample efficiency of the feature extractor. 
Second, it allows the adaptation of the feature extractor to label shift. 
The latter is important because the optimal feature extractor is not necessarily independent of the label distribution. 
% In particular, 
% in generalized label shift, 
The feature transformation $h$ may be unknown, and additional unlabeled test samples can ease the learning of $h$. 

%% what we did in this paper
Thus this paper introduces the \emph{Online Label Shift adaptation with Online Feature Updates} (OLS-OFU) framework, aimed at enhancing feature representation learning in the context of online label shift adaptation. Specifically, each instantiation of OLS-OFU incorporates a self-supervised learning method associated with a loss function denoted as $l_{\rm ssl}$ and an existing online label shift adaptation (OLS) algorithm.
% (i.e., OLS). 
Arbitrarily inserting the feature extractor update into previous OLS algorithms would violate the underlying hypothesis crucial to their performance, and break the theoretical guarantee.
We carefully design OLS-OFU as: in each time step, it executes a modified version of OLS, updates the feature extractor through self-supervised learning, and subsequently refines the last linear prediction layer. 

OLS-OFU is easy to implement and can be seamlessly integrated with any off-the-shelf OLS algorithms.
Theoretically, we demonstrate that OLS-OFU reduces the loss of the overall algorithm by leveraging self-supervised learning techniques to enhance the feature extractor, thereby improving predictions for test samples at each time step $t$. 
Empirical evaluations on CIFAR-10 and CIFAR-10C datasets, considering both online label shift and online generalized label shift scenarios, affirm the effectiveness of OLS-OFU. 
It outperforms its counterpart OLS method across various datasets and distribution shift settings and consistently across all OLS methods, underscoring its robustness. 

%Notably, the advantages of OLS-OFU become particularly pronounced in cases of domain shifts that happened in the generalized label shift.


